Numerical Exploration of Soliton Creation

We explore the classical production of solitons in the easy axis O(3) model in 1+1 dimensions, for a wide range of initial conditions that correspond to the scattering of small breathers. We characterize the fractal nature of the region in parameter space that leads to soliton production and find certain trends in the data. We identify a tension in the initial conditions required for soliton production - low velocity incoming breathers are more likely to produce solitons, while high velocity incoming breathers provide momentum to the final solitons and enable them to separate. We find new "counter-spinning" initial conditions that can alleviate some of this tension.

==> Fit_bvvoq.tex <==
\begin{equation}
\langle v_b \rangle_{\xi}=( -0.15 \pm 0.08 )m_b^2+( 0.86 \pm 0.23 )m_b+( -0.33 \pm 0.17 )
\end{equation}


==> Fit_kvvoq.tex <==
\begin{equation}
\langle v_k \rangle_{v_b,\xi}=( -0.38 \pm 0.19 )m_b^2+( 1.65 \pm 0.55 )m_b+( -1.11 \pm 0.39 )
\end{equation}

